SoK: A Systematic Evaluation of Backdoor Trigger Characteristics in Image Classification

Deep learning achieves outstanding results in many machine learning tasks. Nevertheless, it is vulnerable to backdoor attacks that modify the training set to embed a secret functionality in the trained model. The modified training samples have a secret property, i. e., a trigger. At inference time, the secret functionality is activated when the input contains the trigger, while the model functions correctly in other cases. While there are many known backdoor attacks (and defenses), deploying a stealthy attack is still far from trivial. Successfully creating backdoor triggers depends on numerous parameters. Unfortunately, research has not yet determined which parameters contribute most to the attack performance. This paper systematically analyzes the most relevant parameters for the backdoor attacks, i.e., trigger size, position, color, and poisoning rate. Using transfer learning, which is very common in computer vision, we evaluate the attack on state-of-the-art models (ResNet, VGG, AlexNet, and GoogLeNet) and datasets (MNIST, CIFAR10, and TinyImageNet). Our attacks cover the majority of backdoor settings in research, providing concrete directions for future works. Our code is publicly available to facilitate the reproducibility of our results.

==> ccs_main.tex <==
% CCS format.
%\documentclass[sigconf,review=false,nonacm]{acmart}
% \documentclass[sigconf,review=true,nonacm]{acmart}

%\IEEEoverridecommandlockouts
% The preceding line is only needed to identify funding in the first footnote. If that is unneeded, please comment it out.
\input{preamble}

\begin{document}

\title{A Systematic Evaluation of Backdoor Trigger Characteristics in Image Classification}

% Alternative titles:
% Investigating the Impact of Backdoor Triggers on Image Classification Performance: A Systematic Study

% Characterizing Backdoor Vulnerabilities in Image Classification Systems: A Comprehensive Analysis


\author{Gorka Abad}
\authornote{Authors contributed equally to this research.}
\affiliation{%
  \institution{Radboud University}
  \country{Nijmegen, Netherlands}
}
\affiliation{%
  \institution{Ikerlan research centre}
  \country{Arrasate-Mondragón, Spain}
}
\email{abad.gorka@ru.nl}


\author{Jing Xu}
\authornotemark[1]
\affiliation{%
  \institution{Delft University of Technology}
  \city{Delft}
  \country{Netherlands}}
\email{j.xu-8@tudelft.nl}

\author{Stefanos Koffas}
\authornotemark[1]
\affiliation{
  \institution{Delft University of Technology}
  \city{Delft}
  \country{Netherlands}
}
\email{s.koffas@tudelft.nl}

\author{Behrad Tajalli}
\authornotemark[1]
\affiliation{%
  \institution{Radboud University}
  \country{Nijmegen, Netherlands}
}
\email{hamidreza.tajalli@ru.nl}

\author{Stjepan Picek}
\affiliation{
  \institution{Radboud University}
  \city{Nijmegen}
  \country{Netherlands}
}
\affiliation{
  \institution{Delft University of Technology}
  \city{Delft}
  \country{Netherlands}
}
\email{stjepan.picek@ru.nl}

\begin{abstract}

Deep learning achieves outstanding results in many machine learning tasks. Nevertheless, it is vulnerable to backdoor attacks that modify the training set to embed a secret functionality in the trained model. The modified training samples have a secret property, i. e., a trigger. At inference time, the secret functionality is activated when the input contains the trigger, while the model functions correctly in other cases. While there are many known backdoor attacks (and defenses), deploying a stealthy attack is still far from trivial. Successfully creating backdoor triggers heavily depends on numerous parameters. Unfortunately, research has not yet determined which parameters contribute most to the attack performance.

This paper systematically analyzes the most relevant parameters for the backdoor attacks, i.e., trigger size, position, color, and poisoning rate. Using transfer learning, which is very common in computer vision, we evaluate the attack on numerous state-of-the-art models (ResNet, VGG, AlexNet, and GoogLeNet) and datasets (MNIST, CIFAR10, and TinyImageNet). Our attacks cover the majority of backdoor settings in research, providing concrete directions for future works. Our code is publicly available~\footnote{Code will be shared after paper acceptance.} to facilitate the reproducibility of our results.

\end{abstract}

\begin{CCSXML}
<ccs2012>
   <concept>
       <concept_id>10002978</concept_id>
       <concept_desc>Security and privacy</concept_desc>
       <concept_significance>500</concept_significance>
       </concept>
   <concept>
       <concept_id>10010147.10010257</concept_id>
       <concept_desc>Computing methodologies~Machine learning</concept_desc>
       <concept_significance>500</concept_significance>
       </concept>
 </ccs2012>
\end{CCSXML}

\ccsdesc[500]{Security and privacy}
\ccsdesc[500]{Computing methodologies~Machine learning}

%\begin{IEEEkeywords}
%Backdoor attacks, backdoor trigger, computer vision
%\end{IEEEkeywords}
\keywords{Backdoor attacks, backdoor trigger, computer vision}

\maketitle

\input{sections/1_introduction}
\input{sections/2_background}
\input{sections/2_motivation}
\input{sections/3_threat_model}
\input{sections/4_experiments}
\input{sections/5_related_work.tex}
\input{sections/6_conclusions}

%\clearpage
\bibliography{bibliography}
\bibliographystyle{acmart}

\input{sections/7_appendix}
\end{document}

% ddl: Jan. 19, 2023

==> sections/experiment_matrix.tex <==
\section{Experiment Matrix}
This section describes each factor and associated values and motivates their selection for the present study.



==> sections/experimental_setup.tex <==
\section{Experimental Setup and Results}
\subsection{Experimental Setup}
